High drag states in tidally modulated stratified wakes

Large eddy simulations (LES) are employed to investigate the role of time-varying currents on the form drag and vortex dynamics of submerged 3D topography in a stratified rotating environment. The current is of the form $U_c+U_t \sin(2\pi f_t t)$, where $U_c$ is the mean, $U_t$ is the tidal component and $f_t$ is its frequency. A conical obstacle is considered in the regime of low Froude number. When tides are absent, eddies are shed at the natural shedding frequency $f_{s,c}$. The relative frequency $f^*=f_{s,c}/f_t$ is varied in a parametric study which reveals states of high time-averaged form drag coefficient. There is a two-fold amplification of the form drag coefficient relative to the no-tide ($U_t=0$) case when $f^*$ lies between 0.5 and 1. The spatial organization of the near-wake vortices in the high drag states is different from a K\'arm\'an vortex street. For instance, the vortex shedding from the obstacle is symmetric when $f^*=5/12$ and strongly asymmetric when $f^*=5/6$. The increase in form drag with increasing $f^*$ stems from bottom intensification of the pressure in the obstacle lee which is linked to changes in flow separation and near-wake vortices.

==> Introduction.tex <==
The role of bottom topography in ocean dynamics   has received increasing attention in recent years. 
%  Rough topography   enhances bottom drag on oceanic flows  and also promotes turbulent mixing of the interior fluid. 
% Internal waves are launched when currents and tides  flow over sloping topography. 
 The momentum transported by topographic  internal waves  act as drag on the impinging flow, and the energy converted from the flow to internal waves acts as  a source for both remote and local turbulent mixing.
